RegionViT: Regional-to-Local Attention for Vision Transformers

Vision transformer (ViT) has recently shown its strong capability in achieving comparable results to convolutional neural networks (CNNs) on image classification. However, vanilla ViT simply inherits the same architecture from the natural language processing directly, which is often not optimized for vision applications. Motivated by this, in this paper, we propose a new architecture that adopts the pyramid structure and employ a novel regional-to-local attention rather than global self-attention in vision transformers. More specifically, our model first generates regional tokens and local tokens from an image with different patch sizes, where each regional token is associated with a set of local tokens based on the spatial location. The regional-to-local attention includes two steps: first, the regional self-attention extract global information among all regional tokens and then the local self-attention exchanges the information among one regional token and the associated local tokens via self-attention. Therefore, even though local self-attention confines the scope in a local region but it can still receive global information. Extensive experiments on four vision tasks, including image classification, object and keypoint detection, semantics segmentation and action recognition, show that our approach outperforms or is on par with state-of-the-art ViT variants including many concurrent works. Our source codes and models are available at https://github.com/ibm/regionvit.

==> Tables/ablation_study/abl_all.tex <==
\begin{table}[b]
    \centering
    \caption{{Ablation Study.} \ours-S is used as baseline.}
    \label{table:abl_all}
    \begin{subtable}[h]{0.48\textwidth}
        \subimport{./}{Tables/ablation_study/abl_downsample}
    \end{subtable}
    \quad
    % \begin{subtable}[h]{0.31\textwidth}
    %     \subimport{./}{Tables/ablation_study/abl_window_size}
    % \end{subtable}
    % \begin{subtable}[h]{0.45\textwidth}
    % \subimport{./}{Tables/ablation_study/abl_regional_tokens}
    % \end{subtable}
    % \quad
    \begin{subtable}[h]{0.48\textwidth}
        \subimport{./}{Tables/ablation_study/abl_rel_pos}
    \end{subtable}
\end{table}

==> Tables/ablation_study/abl_window_size.tex <==
% \begin{table}[t]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{cccc}
        \toprule
        Window Sizes & Params (M) & FLOPs (G) & IN1K Acc. (\%) \\
        \midrule
        28 & 34.1 & 6.7 & OOM \\
        14 & 31.3 & 5.7 & 83.2 \\
        7 & 30.6 & 5.3 & 82.6 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \vspace{-2mm}
    \caption{\scriptsize{Different window size for local tokens.}}
    \label{table:abl_window_size}
% \end{table}

==> Tables/detection_all.tex <==
\begin{table}[ht]
\begin{center}
\caption{Object detection performance on the COCO val2017 with RetinaNet. \rc{Current results are not optimized, need more tuning}}
\label{table:det_retinanet}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Backbone} & Params & FLOPs & \multicolumn{6}{c|}{RetinaNet 1x schedule} & \multicolumn{6}{c}{RetinaNet 3x + MS schedule}\\
& (M) & (G) & $AP$ & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ & $AP$ & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ \\
\midrule
% ResNet18 & 21.3 & 190.33 & 31.8 & 49.6 & 33.6 & 16.3 & 34.3 & 43.2 & 35.4 & 53.9 & 37.6 & 19.5 & 38.2 & 46.8 \\
% PVT-T~\cite{PVT_wang2021} & 23.0 & n/a & 36.7 & 56.9 & 38.9 & 22.6 & 38.8 & 50.0 & 39.4 & 59.8 & 42.0 & 25.5 & 42.0 & 52.1 \\
% % https://ml.azure.com/experiments/msvit_det-c4cc9a53/runs/msvit_det-c4cc9a53-retina_msvit_tiny_lr1e-4_qkvbiastrue_scus-trainval_retinanet_with_msvit_widemedim_lr1e-4_wd0_1_bsz16-160385b0?wsid=/subscriptions/8d7c0a6f-7c2e-4e4b-becf-f9ee95433147/resourcegroups/Image_Languge_Pretraining-aml/workspaces/Image_Languge_Pretraining-aml
% % max_mem: 7167M
% % \rowcolor{Graylight} 
% ViL-T~\cite{ViL_Zhang_2021tu} & 16.6 & 171.91 & 38.8 & 59.0 & 41.3 & 23.8 & 41.5 & 51.8 & 40.7 & 61.2 & 43.2 & 26.4 & 43.9 & 53.6 \\
% \midrule
ResNet50 & 37.7 & 239.3 & 36.3 & 55.3 & 38.6 & 19.3 & 40.0 & 48.8 & 39.0 & 58.4 & 41.8 & 22.4 & 42.8 & 51.6 \\
PVT-S~\cite{PVT_wang2021} & 34.2 & $-$ & 40.4 & 61.3 & 43.0 & 25.0 & 42.9 & 55.7 & 42.2 & 62.7 & 45.0 & 26.2 & 45.2 & 57.2\\
% https://ml.azure.com/experiments/msvit_det-9f976a33/runs/msvit_det-9f976a33-retina_msvit_small_lr1e-4_smallwd_qkvbiastrue-trainval_retinanet_with_msvit_small_wd5e-2-2049f92b?wsid=/subscriptions/46da6261-2167-4e71-8b0d-f4a45215ce61/resourcegroups/researchvc-sea/workspaces/resrchvc-sea
% 1300M
% \rowcolor{Graylight} 
ConT-M~\cite{ConT_Yan_2021vn} & 27.0 & 217.2 & 39.3 & 59.3 & 41.8 & 23.1 & 43.1 & 51.9 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
ViL-S~\cite{ViL_Zhang_2021tu} & 35.7 & 252.2 & 41.6 & 62.5 & 44.1 & 24.9 & 44.6 & 56.2 & 42.9 & 63.8 & 45.6 & 27.8 & 46.4 & 56.3 \\
Twins-SVT-S~\cite{Twins_Chu_2021to} & 34.3 & 209 & 42.3 & 63.4 & 45.2 & 26.0 & 45.5 & 56.5 \\
% \ours-Ti & 40.8 & 295.5 & 42.6784 & 64.6715 & 45.5532 & 28.9995 & 46.7246 & 54.4370 & 42.6352 & 63.5731 & 45.3925 & 27.2653 & 45.6553 & 55.6137 \\ % trained with ms for both schedule, and freeze at 2 without dp and high weight decay
% \ours-Ti+ & 41.2 & 316.6 & 42.6784 & 64.6715 & 45.5532 & 28.9995 & 46.7246 & 54.4370 & 42.6352 & 63.5731 & 45.3925 & 27.2653 & 45.6553 & 55.6137 \\

\midrule
ResNet101 & 56.7 & 319.1 & 38.5 & 57.8 & 41.2 & 21.4 & 42.6 & 51.1 & 40.9 & 60.1 & 44.0 & 23.7 & 45.0 & 53.8 \\
ResNeXt101-32x4d & 56.4 & 319.1 & 39.9 & 59.6 & 42.7 & 22.3 & 44.2 & 52.5 & 41.4 & 61.0 & 44.3 & 23.9 & 45.5 & 53.7 \\
PVT-M~\cite{PVT_wang2021} & 53.9 & $-$ & 41.9 & 63.1 & 44.3 & 25.0 & 44.9 & 57.6 & 43.2 & 63.8 & 46.1 & 27.3 & 46.3 & 58.9 \\

% https://ml.azure.com/job/Image_Languge_Pretraining/az-scus-v100-2/111e3a7b1cf47eb9330abb66817e3bfc
% max_mem: 20530M
% \rowcolor{Graylight} 
ViL-M~\cite{ViL_Zhang_2021tu} & 50.8 & 338.9 & 42.9 & 64.0 & 45.4 & 27.0 & 46.1 & 57.2 & 43.7 & 64.6 & 46.4 & 27.9 & 47.1 & 56.9 \\
\rowcolor{Gray}
\ours-Ti & 40.8 & 295.5 & 42.1 & 64.5 & 45.1 & 27.0 & 44.6 & 55.0 \\
\rowcolor{Gray}
\ours-Ti+ & 41.5 & 315.6 & 43.0 & 65.2 & 45.8 & 28.3 & 45.6 & 56.9    \\
\midrule
ResNeXt101-64x4d & 95.5 & 483.6 & 41.0 & 60.9 & 44.0 & 23.9 & 45.2 & 54.0 & 41.8 & 61.5 & 44.4 & 25.2 & 45.4 & 54.6 \\
PVT-L~\cite{PVT_wang2021} & 71.1 & $-$ & 42.6 & 63.7 & 45.4 & 25.8 & 46.0 & 58.4 & 43.4 & 63.6 & 46.1 & 26.1 & 46.0 & 59.5 \\
% https://ml.azure.com/experiments/msvit_det-c4cc9a53/runs/msvit_det-c4cc9a53-retina_msvit_base_lr8e-5_qkvbiastrue-trainval_retinanet_with_msvit_deepbase_lr8e-5_wd0_15-2c10da1b?wsid=/subscriptions/46da6261-2167-4e71-8b0d-f4a45215ce61/resourcegroups/msrhyperVC/workspaces/msrhyper
% max_mem: 21456M
% \rowcolor{Graylight} 
ViL-B~\cite{ViL_Zhang_2021tu} & 66.7 & 443.0 & 44.3 & 65.5 & 47.1 & 28.9 & 47.9 & 58.3 & 44.7 & 65.5 & 47.6 & 29.9 & 48.0 & 58.1 \\
Twins-SVT-B~\cite{Twins_Chu_2021to} & 67.0 & 322 & 44.4 & 65.8 & 47.4 & 27.9 & 47.8 & 59.5 \\
Twins-SVT-L~\cite{Twins_Chu_2021to} & 110.9 & 455 & 44.8 & 66.1 & 48.1 & 28.4 & 48.3 & 60.1 \\
\rowcolor{Gray}
\ours-M & 51.4 & 352.5 & 42.2 & 64.2 & 45.3 & 28.4 & 44.3 & 55.7\\
\rowcolor{Gray}
\ours-M+ & 52.2 & 377.0 & 43.5 & 65.8 & 46.6 & 29.2 & 45.4 & 57.8\\
\rowcolor{Gray}
\ours-B & 83.4 & 495.1 & 43.0 & 65.2 & 46.3 & 28.8 & 45.1 & 56.3   \\
\rowcolor{Gray}
\ours-B+ & 84.5 & 536.2 &  44.1 & 66.4 & 47.5 & 29.2 & 45.9 & 58.4  \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

\begin{table}[ht]
\begin{center}
\caption{Object detection and instance segmentation performance on the COCO val2017 with Mask R-CNN.}
\label{table:det_maskrcnn}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Backbone} & Params & FLOPs & \multicolumn{6}{c|}{Mask R-CNN 1x schedule} & \multicolumn{6}{c}{Mask R-CNN 3x + MS schedule}\\
 & (M) & (G) & $AP^b$ & $AP^b_{50}$ & $AP^b_{75}$ & $AP^m$ & $AP^m_{50}$ & $AP^m_{75}$ & $AP^b$ & $AP^b_{50}$ & $AP^b_{75}$ & $AP^m$ & $AP^m_{50}$ & $AP^m_{75}$ \\
\midrule

% ResNet18 & 31.2 & 131.03 & 34.0 & 54.0 & 36.7 & 31.2 & 51.0 & 32.7 & 36.9 & 57.1 & 40.0 & 33.6 & 53.9 & 35.7\\
% PVT-T~\cite{PVT_wang2021} & 32.9 & $-$ & 36.7 & 59.2 & 39.3 & 35.1 & 56.7 & 37.3 & 39.8 & 62.2 & 43.0 & 37.4 & 59.3 & 39.9 \\
% % \rowcolor{Graylight} 
% ViL-T~\cite{ViL_Zhang_2021tu} & 26.9 & 94.3 & 38.7 & 61.1 & 41.3 & 36.2 & 58.3 & 38.2 & 41.2 & 63.0 & 44.7 & 37.9 & 59.8 & 40.6 \\
% % https://ml.azure.com/job/resrchvc/az-eus-v100-16gb-2/36255ae140052573c1ea521dacf90440
% \midrule
ResNet50 & 44.2 & 180.0 & 38.0 & 58.6 & 41.4 & 34.4 & 55.1 & 36.7 & 41.0 & 61.7 & 44.9 & 37.1 & 58.4 & 40.1 \\
ConT-M~\cite{ConT_Yan_2021vn} & $-$ & $-$ & 40.5 & $-$ & $-$ & 38.1 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
PVT-S~\cite{PVT_wang2021} & 44.1 & $-$ & 40.4 & 62.9 & 43.8 & 37.8 & 60.1 & 40.3 & 43.0 & 65.3 & 46.9 & 39.9 & 62.5 & 42.8 \\
% \rowcolor{Graylight} 
Twins-SVT-S~\cite{Twins_Chu_2021to} & 44.0 & 228 & 42.7 & 65.6 & 46.7 & 39.6 & 62.5 & 42.6 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\

ViL-S~\cite{ViL_Zhang_2021tu} & 45.0 & 174.3 & 41.8 & 64.1 & 45.1 & 38.5 & 61.1 & 41.4 & 43.4 & 64.9 & 47.0 & 39.6 & 62.1 & 42.4 \\
% \ours-Ti & 50.1 & 259.1 & 42.7418 & 66.0848 & 46.6344 & 39.7105 & 63.1229 & 42.3239 & 43.7050 & 65.5401 & 47.5571 & 40.0263 & 62.6961 & 42.7916\\

% https://ml.azure.com/job/gcrprojvc1/az-wus2-v100-32gb-3/1378be65b7aa1c206bfa74226a38c86a
% exp: https://ml.azure.com/job/gcrprojvc1/az-wus2-v100-32gb-3/6c2b53df6881b2866f3bfaf056b52c6f
% https://ml.azure.com/job/gcrprojvc1/az-wus2-v100-32gb-3/e37f414585c5d86cac795cab230d1ead
\midrule
ResNet101 & 63.2 & 259.8  & 40.4 & 61.1 & 44.2 & 36.4 & 57.7 & 38.8 & 42.8 & 63.2 & 47.1 & 38.5 & 60.1 & 41.3 \\
ResNeXt101-32x4d & 62.8 & 259.8 & 41.9 & 62.5 & 45.9 & 37.5 & 59.4 & 40.2 & 44.0 & 64.4 & 48.0 & 39.2 & 61.4 & 41.9 \\
PVT-M~\cite{PVT_wang2021} & 63.9 & $-$ & 42.0 & 64.4 & 45.6 & 39.0 & 61.6 & 42.1 & 44.2 & 66.0 & 48.2 & 40.5 & 63.1 & 43.5 \\

ViL-M~\cite{ViL_Zhang_2021tu} & 60.1 & 261.1 & 43.4 & 65.9 & 47.0 & 39.7 & 62.8 & 42.1 & 44.6 & 66.3 & 48.5 & 40.7 & 63.8 & 43.7 \\
% https://ml.azure.com/job/gcrprojvc1/az-wus2-v100-32gb-3/13f2aa35db37c75657fb997ad0be18b8
\rowcolor{Gray}
\ours-Ti & 50.1 & 259.1 & 42.0 & 65.5 & 45.7 & 39.1 & 62.5 & 41.9 & \\
\rowcolor{Gray}
\ours-Ti+ & 50.9 & 279.1 & 42.9 & 66.4 & 47.0 & 40.0 & 63.5 & 42.9 \\

\midrule
ResNeXt101-64x4d & 101.9 & 424.3 & 42.8 & 63.8 & 47.3 & 38.4 & 60.6 & 41.3 & 44.4 & 64.9 & 48.8 & 39.7 & 61.9 & 42.6 \\
PVT-L~\cite{PVT_wang2021} & 81.0 & $-$ & 42.9 & 65.0 & 46.6 & 39.5 & 61.9 & 42.5 & 44.5 & 66.0 & 48.3 & 40.7 & 63.4 & 43.7 \\
% \rowcolor{Graylight} 
ViL-B~\cite{ViL_Zhang_2021tu} & 76.1 & 365.1 & 45.1 & 67.2 & 49.3 & 41.0 & 64.3 & 44.2 & 45.7 & 67.2 & 49.9 & 41.3 & 64.4 & 44.5 \\
Twins-SVT-B~\cite{Twins_Chu_2021to} & 76.3 & 340 & 45.1 & 67.0 & 49.4 & 41.1 & 64.1 & 44.4 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
Twins-SVT-L~\cite{Twins_Chu_2021to} & 119.7 & 474 & 45.2 & 67.5 & 49.4 & 41.2 & 64.5 & 44.5 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
\rowcolor{Gray}
\ours-M & 60.7 & 313.6 & 41.9 & 65.5 & 45.7 & 39.2 & 62.4 & 41.9 \\
\rowcolor{Gray}
\ours-M+ & 61.6 & 340.5 & 43.1 & 66.6 & 47.0 & 40.2 & 63.7 & 42.9 \\

\rowcolor{Gray}
\ours-B & 92.1 & 459.0 &  42.8 & 67.1 & 46.9 & 40.1 & 64.0 & 42.8   \\
\rowcolor{Gray}
\ours-B+ & 93.2 & 500.1 &  44.0 & 68.2 & 48.5 & 41.2 & 65.1 & 44.3  \\


% https://ml.azure.com/job/msrhyper/msr-lab-hyper-dgx2/ad92391242af8a3560c8c6be6f57c732
% https://ml.azure.com/job/msrhyper/msr-lab-hyper-dgx2/49f8a2e7359ef8a071f64125640f176d
% https://ml.azure.com/experiments/msvit_det-c4cc9a53/runs/msvit_det-c4cc9a53-maskrcnn_msvit_base_lr1e-4_largewd_qkvbiastrue-trainval_maskrcnn_with_msvit_large_sparse_attn_avg_token_no_freeze_backbonelr1_0_1e-4_wd1e-1-e47153d1?wsid=/subscriptions/46da6261-2167-4e71-8b0d-f4a45215ce61/resourcegroups/msrhyperVC/workspaces/msrhyper
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}


==> Tables/detection_bk.tex <==
\begin{table}[ht]
\centering
\caption{Object detection performance on the COCO val2017 with 1$\times$ schedule.}
\label{table:detection}
\begin{subtable}[h]{0.48\textwidth}  % RetinaNet
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c|c|c|c|c|c}
\toprule
Backbone & Params (M) & FLOPs (G) & $AP$ & $AP_{50}$ & $AP_{75}$ & $AP_{S}$ & $AP_{M}$ & $AP_{L}$ \\
\midrule
ResNet50 & 37.7 & 234 & 36.3 & 55.3 & 38.6 & 19.3 & 40.0 & 48.8  \\
ConT-M~\cite{ConT_Yan_2021vn} & 27.0 & 217.2 & 39.3 & 59.3 & 41.8 & 23.1 & 43.1 & 51.9  \\
PVT-S~\cite{PVT_wang2021} & 34.2 & $-$ & 40.4 & 61.3 & 43.0 & 25.0 & 42.9 & 55.7\\
% Twins-SVT-S~\cite{Twins_Chu_2021to} & 34.3 & 209 & 42.3 & 63.4 & 45.2 & 26.0 & 45.5 & 56.5 \\
ViL-S~\cite{ViL_Zhang_2021tu} & 35.7 & 252.2 & 41.6 & 62.5 & 44.1 & 24.9 & 44.6 & 56.2 \\
Swin-T~\cite{Swin_Liu_2021tq} & 38.5 & 245 & 41.5 & 62.1 &  44.2 & 25.1 & 44.9 & 55.5 \\
Twins-SVT-S (w/ PEG)~\cite{Twins_Chu_2021to} & 34.3 & 209 & 43.0 & 64.2 & 46.3 & 28.0 & 46.4 & 57.5 \\
\rowcolor{Gray}
% \ours-Ti & 40.8 & 295.5 & 42.1 & 64.5 & 45.1 & 27.0 & 44.6 & 55.0 \\
\ours-Ti & 40.8 & 192.6 & 42.1 & 63.8 & 45.2 & 26.6 & 45.9 & 54.8 \\
% \rowcolor{Gray}
% \ours-Ti w/ PEG & 40.8 & 192.6 & 43.3 & 65.0 & 46.6 & 27.5 & 47.0 & 57.0 \\
\rowcolor{Gray}
% \ours-Ti+ & 41.5 & 315.6 & 43.0 & 65.2 & 45.8 & 28.3 & 45.6 & 56.9   \\
\ours-Ti+ & 41.5 & 204.2 & 43.1 & 65.1 & 46.1 & 28.4 & 46.3 & 56.9   \\
\rowcolor{Gray}
\ours-Ti+ w/ PEG & 41.6 & 204.3 & 43.4 & 65.5 & 46.2 & 27.9 & 47.2 & 56.8   \\  % 43.7 & 65.5 & 46.8 & 29.3 & 47.1 & 57.3
\midrule
ResNet101 & 56.7 & 315 & 38.5 & 57.8 & 41.2 & 21.4 & 42.6 & 51.1 \\
ResNeXt101-32x4d & 56.4 & 319.1 & 39.9 & 59.6 & 42.7 & 22.3 & 44.2 & 52.5 \\
PVT-M~\cite{PVT_wang2021} & 53.9 & $-$ & 41.9 & 63.1 & 44.3 & 25.0 & 44.9 & 57.6  \\
ViL-M~\cite{ViL_Zhang_2021tu} & 50.8 & 338.9 & 42.9 & 64.0 & 45.4 & 27.0 & 46.1 & 57.2 \\
Swin-S~\cite{Swin_Liu_2021tq} & 59.8 & 335 & 44.5 & 65.7 & 47.5 & 27.4 & 48.0 & 59.9 \\
Twins-SVT-B (w/ PEG)~\cite{Twins_Chu_2021to} & 67.0 & 322 & 45.3 & 66.7 & 48.1 & 28.5 & 48.9 & 60.6 \\
% \ours-B & 83.4 & 495.1 & 43.0 & 65.2 & 46.3 & 28.8 & 45.1 & 56.3   \\
\rowcolor{Gray}
\ours-B & 83.4 & 308.9 & 43.2 & 65.1 & 46.3 & 29.7 & 46.6 & 56.8  \\
% \rowcolor{Gray}
% \ours-B w/ PEG & 83.4 & 309 &  44.1 & 66.0 & 47.1 & 29.4 & 47.6 & 57.6 \\
\rowcolor{Gray}
% \ours-B+ & 84.5 & 536.2 & 44.1 & 66.4 & 47.5 & 29.2 & 45.9 & 58.4  \\
\ours-B+ & 84.4 & 328.1 & 44.2 & 66.3 & 47.3 & 29.1 & 47.4 & 58.8  \\
\rowcolor{Gray}
\ours-B+ w/ PEG & 84.5 & 328.2 & 44.6 & 66.4 & 47.7 & 28.7 & 47.9 & 59.1  \\
\midrule
ResNeXt101-64x4d & 95.5 & 473 & 41.0 & 60.9 & 44.0 & 23.9 & 45.2 & 54.0 \\
PVT-L~\cite{PVT_wang2021} & 71.1 & 345 & 42.6 & 63.7 & 45.4 & 25.8 & 46.0 & 58.4 \\
ViL-B~\cite{ViL_Zhang_2021tu} & 66.7 & 443.0 & 44.3 & 65.5 & 47.1 & 28.9 & 47.9 & 58.3 \\
Swin-B~\cite{Swin_Liu_2021tq} & 98.4 & 477 & 44.7 & 65.9 & 49.2 & $-$ & $-$ & $-$ \\
Twins-SVT-L (w/ PEG)~\cite{Twins_Chu_2021to} & 110.9 & 455 & 45.7 & 67.1 & 49.2 & $-$ & $-$ & $-$ \\
% Twins-SVT-B~\cite{Twins_Chu_2021to} & 67.0 & 322 & 44.4 & 65.8 & 47.4 & 27.9 & 47.8 & 59.5 \\
% Twins-SVT-L~\cite{Twins_Chu_2021to} & 110.9 & 455 & 44.8 & 66.1 & 48.1 & 28.4 & 48.3 & 60.1 \\
% \rowcolor{Gray}
% \ours-M & 51.4 & 352.5 & 42.2 & 64.2 & 45.3 & 28.4 & 44.3 & 55.7\\
% \rowcolor{Gray}
% \ours-M+ & 52.2 & 377.0 & 43.5 & 65.8 & 46.6 & 29.2 & 45.4 & 57.8\\
\rowcolor{Gray}
\ours-B+ w/ PEG$\dagger$ & 84.5 & 506.4 & 45.6 & 67.6 & 49.0 & 31.4 & 48.9 & 59.6 \\
\bottomrule
\multicolumn{9}{l}{\footnotesize The results of Swin~\cite{Swin_Liu_2021tq} is copied from Twins~\cite{Twins_Chu_2021to} as the original paper does not include resutls with ImageNet1K weights.} \\
\multicolumn{9}{l}{\footnotesize $\dagger$: input resolution is 896$\times$1344.}
\end{tabular}
\end{adjustbox}
\caption{RetinaNet.}
\label{table:det_retinanet}

\end{subtable}
\quad
\begin{subtable}[h]{0.48\textwidth}  % MaskRCNN
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l@{\hspace{3pt}}|c@{\hspace{3pt}}|c|c|c|c|c|c|c}
\toprule
Backbone & Params (M) & FLOPs (G) & $AP^b$ & $AP^b_{50}$ & $AP^b_{75}$ & $AP^m$ & $AP^m_{50}$ & $AP^m_{75}$\\
\midrule
ResNet50 & 44.2 & 260.0 & 38.0 & 58.6 & 41.4 & 34.4 & 55.1 & 36.7 \\
ConT-M~\cite{ConT_Yan_2021vn} & $-$ & $-$ & 40.5 & $-$ & $-$ & 38.1 \\
PVT-S~\cite{PVT_wang2021} & 44.1 & $-$ & 40.4 & 62.9 & 43.8 & 37.8 & 60.1 & 40.3  \\
% \rowcolor{Graylight} 
% Twins-SVT-S~\cite{Twins_Chu_2021to} & 44.0 & 228 & 42.7 & 65.6 & 46.7 & 39.6 & 62.5 & 42.6 \\
ViL-S~\cite{ViL_Zhang_2021tu} & 45.0 & 174.3 & 41.8 & 64.1 & 45.1 & 38.5 & 61.1 & 41.4  \\
% \ours-Ti & 50.1 & 259.1 & 42.0 & 65.5 & 45.7 & 39.1 & 62.5 & 41.9 \\
Swin-T~\cite{Swin_Liu_2021tq} & 47.8 & 264 & 42.2 & 64.6 & 46.2 & 39.1 & 61.6 & 42.0 \\
Twins-SVT-S (w/ PEG)~\cite{Twins_Chu_2021to} & 44.0 & 228 & 43.5 & 66.0 & 47.3 & 40.3 & 63.2 & 43.4 \\
\rowcolor{Gray}
\ours-Ti & 50.1 & 171.3 & 42.2 & 65.2 & 46.0 & 39.0 & 62.0 & 41.5 \\
% \rowcolor{Gray}
% \ours-Ti w/ PEG & 50.1 & 171.3 & 43.3 & 66.0 & 47.2 & 40.0 & 63.2 & 42.7 \\
% \ours-Ti+ & 50.9 & 279.1 & 42.9 & 66.4 & 47.0 & 40.0 & 63.5 & 42.9 \\
\rowcolor{Gray}
\ours-Ti+ & 50.9 & 182.9 & 43.0 & 66.0 & 46.8 & 39.8 & 63.0 & 42.8 \\
\rowcolor{Gray}
\ours-Ti+ w/ PEG & 50.9 & 183.0 & 44.2 & 67.2 & 48.2 & 40.6 & 63.9 & 43.6 \\
\midrule
ResNet101 & 63.2 & 336  & 40.4 & 61.1 & 44.2 & 36.4 & 57.7 & 38.8  \\
ResNeXt101-32x4d & 62.8 & 340 & 41.9 & 62.5 & 45.9 & 37.5 & 59.4 & 40.2 \\
PVT-M~\cite{PVT_wang2021} & 63.9 & $-$ & 42.0 & 64.4 & 45.6 & 39.0 & 61.6 & 42.1 \\
ViL-M~\cite{ViL_Zhang_2021tu} & 60.1 & 261.1 & 43.4 & 65.9 & 47.0 & 39.7 & 62.8 & 42.1 \\
Swin-S~\cite{Swin_Liu_2021tq} & 69.1 & 354 & 44.8 & 66.6 & 48.9 & 40.9 & 63.4 & 44.2 \\
Twins-SVT-B (w/ PEG)~\cite{Twins_Chu_2021to} & 76.3 & 340 & 45.2 & 67.6 & 49.3 & 41.5 & 64.5 & 44.8  \\
% \ours-B & 92.1 & 459.0 &  42.8 & 67.1 & 46.9 & 40.1 & 64.0 & 42.8   \\
\rowcolor{Gray}
\ours-B & 92.2 & 287.9 & 42.8 & 65.6 & 46.3 & 39.5 & 62.6 & 42.2   \\
% \rowcolor{Gray}
% \ours-B w/ PEG & 92.2 & 288.0 & 44.2 & 66.7 & 48.4 & 40.4 & 63.5 & 43.3 \\
\rowcolor{Gray}
\ours-B+ & 93.2 & 307.1 &  43.9 & 66.7 & 47.9 & 40.2 & 63.6 & 43.0 \\
\rowcolor{Gray}
\ours-B+ w/ PEG & 93.2 & 307.2 & 44.7 & 67.3 & 49.1 & 40.9 & 64.1 & 44.1 \\
\midrule
ResNeXt101-64x4d & 101.9 & 493 & 42.8 & 63.8 & 47.3 & 38.4 & 60.6 & 41.3 \\
PVT-L~\cite{PVT_wang2021} & 81.0 & 364 & 42.9 & 65.0 & 46.6 & 39.5 & 61.9 & 42.5 \\
% \rowcolor{Graylight} 
ViL-B~\cite{ViL_Zhang_2021tu} & 76.1 & 365.1 & 45.1 & 67.2 & 49.3 & 41.0 & 64.3 & 44.2 \\
Swin-B~\cite{Swin_Liu_2021tq} & 107.2 & 496 & 45.5 & $-$ & $-$ & 41.3 & $-$ & $-$ \\
Twins-SVT-L (w/ PEG)~\cite{Twins_Chu_2021to} & 119.7 & 474 & 45.9 & $-$ & $-$ & 41.6 & $-$ & $-$  \\
% Twins-SVT-B~\cite{Twins_Chu_2021to} & 76.3 & 340 & 45.1 & 67.0 & 49.4 & 41.1 & 64.1 & 44.4  \\
% Twins-SVT-L~\cite{Twins_Chu_2021to} & 119.7 & 474 & 45.2 & 67.5 & 49.4 & 41.2 & 64.5 & 44.5  \\
% \rowcolor{Gray}
% \ours-M & 60.7 & 313.6 & 41.9 & 65.5 & 45.7 & 39.2 & 62.4 & 41.9 \\
% \rowcolor{Gray}
% \ours-M+ & 61.6 & 340.5 & 43.1 & 66.6 & 47.0 & 40.2 & 63.7 & 42.9 \\

\rowcolor{Gray}
% \ours-B+ & 93.2 & 500.1 &  44.0 & 68.2 & 48.5 & 41.2 & 65.1 & 44.3  \\
\ours-B+ w/ PEG$\dagger$ & 93.2 & 464.4 & 45.4 & 67.9 & 49.9 & 41.5 & 65.1 & 44.4  \\


% https://ml.azure.com/job/msrhyper/msr-lab-hyper-dgx2/ad92391242af8a3560c8c6be6f57c732
% https://ml.azure.com/job/msrhyper/msr-lab-hyper-dgx2/49f8a2e7359ef8a071f64125640f176d
% https://ml.azure.com/experiments/msvit_det-c4cc9a53/runs/msvit_det-c4cc9a53-maskrcnn_msvit_base_lr1e-4_largewd_qkvbiastrue-trainval_maskrcnn_with_msvit_large_sparse_attn_avg_token_no_freeze_backbonelr1_0_1e-4_wd1e-1-e47153d1?wsid=/subscriptions/46da6261-2167-4e71-8b0d-f4a45215ce61/resourcegroups/msrhyperVC/workspaces/msrhyper
\bottomrule
\multicolumn{9}{l}{\footnotesize The results of Swin~\cite{Swin_Liu_2021tq} is copied from Twins~\cite{Twins_Chu_2021to} as the original paper does not include resutls with ImageNet1K weights.} \\
\multicolumn{9}{l}{\footnotesize $\dagger$: input resolution is 896$\times$1344.}
\end{tabular}
\end{adjustbox}
\caption{Mask R-CNN.}
\label{table:det_maskrcnn}

\end{subtable}


\end{table}

